Localization of Synthetic Manipulations in Western Blot Images

Recent breakthroughs in deep learning and generative systems have significantly fostered the creation of synthetic media, as well as the local alteration of real content via the insertion of highly realistic synthetic manipulations. Local image manipulation, in particular, poses serious challenges to the integrity of digital content and societal trust. This problem is not only confined to multimedia data, but also extends to biological images included in scientific publications, like images depicting Western blots. In this work, we address the task of localizing synthetic manipulations in Western blot images. To discriminate between pristine and synthetic pixels of an analyzed image, we propose a synthetic detector that operates on small patches extracted from the image. We aggregate patch contributions to estimate a tampering heatmap, highlighting synthetic pixels out of pristine ones. Our methodology proves effective when tested over two manipulated Western blot image datasets, one altered automatically and the other manually by exploiting advanced AI-based image manipulation tools that are unknown at our training stage. We also explore the robustness of our method over an external dataset of other scientific images depicting different semantics, manipulated through unseen generation techniques.

==> 2_problem.tex <==
% \section{Problem Formulation}
% \label{sec:problem}
% This paper proposes a method to localize the presence of synthetically generated content within pristine scientific images. 
% % In this section, we provide a formal definition of the problem.
% % The synthetic image detection task consists of discerning whether a given image $\mathbf{I}$ is pristine or artificial. This typically involves to associate to $\mathbf{I}$ a label $y$ as follows:
% % \begin{equation}
% % y = 
% % \begin{cases} 
% % 1 & \text{if } \mathbf{I} \text{ is synthetic} \\
% % 0 & \text{if } \mathbf{I} \text{ is pristine}. 
% % \end{cases}
% % \end{equation}
% % Our goal departs from this traditional scenario since in our case, $\mathbf{I}$ contains both genuine and manipulated regions. 
% %In this context, it is crucial not only to detect whether an image has been manipulated but also to localize the specific areas of tampering within the image.
% % Therefore, we address the two-fold task of tampering detection and localization in a joint fashion.
% Let us consider a manipulated image $\Ibar$ with size $R \times C$, that presents a tampered with region $\mathcal{T}$. We can associate $\Ibar$ with a tampering mask $\mathbf{M}$ of size $R \times C$; $\mathbf{M}$ is a 2D binary matrix where each pixel takes a value of 0 if the corresponding pixel in $\Ibar$ is pristine and a value of 1 if the pixel is synthetic:
% \begin{equation}
%     \label{eq:tampering-mask}
%     \mathbf{M}(r,c) =
%     \begin{cases}
%       1 & \text{if}\ (r,c) \in \mathcal{T} \\
%       0 & \text{otherwise}.
%     \end{cases}  
% \end{equation}

% Our aim is to return a real-valued
% %the tampering mask $\mathbf{M}$ by computing a 
% tampering heatmap $\mathbf{H}$, 
% % Pixel values for $\mathbf{H}$ are defined as follows:
% % \begin{equation}
% %     \label{eq:heatmap}
% %     \mathbf{H}(r,c) = P\left((r,c) \in \mathcal{T} \mid \mathbf{I}_\text{tmp}\right). \textcolor{red}{lowercase P?}
% % \end{equation}
% which differentiates between real and synthetic regions, providing for each pixel the probability of it being synthetically generated. 


